Predictive Network Configuration with Hierarchical Spectral Clustering for Software Defined Vehicles

The increasing connectivity and autonomy of vehicles has led to a growing need for dynamic and real-time adjustments to software and network configurations. Software Defined Vehicles (SDV) have emerged as a potential solution to adapt to changing user needs with continuous updates and onboard reconfigurations to offer infotainment, connected, and background services such as cooperative driving. However, network configuration management in SDVs remains a significant challenge, particularly in the context of shared Ethernet-based in-vehicle networks. Traditional worst-case static configuration methods cannot efficiently allocate network resources while ensuring Quality of Service (QoS) guarantees for each network flow within the physical topology capabilities. In this work, we propose a configuration generation methodology that addresses these limitations by dynamically switching between pre-computed offboard configurations downloaded to the vehicle. Simulation results are presented and future work is discussed.

==> sections/99_old.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{assets/revolutions.pdf}
%     \caption{The evolution of automotive use cases, feature integration, and software complexity. The integration of new features into existing architecture paradigms becomes increasingly difficult (blue curve). The transition to new paradigms and architectures, although extremely demanding in efforts to the entire industry, unlocks the integration of new use cases (black curve).}
%     \label{fig:revolutions}
% \end{figure}

% \section{Thesis objectives}
% In this PhD, we aim to define the missing infrastructure layer in order to propose this full architecture as the next automotive paradigm. The planned steps are:

% \begin{enumerate}
%     \item \textbf{Survey (in progress):} First, we cover the current literature in other relevant industries to serve as inspiration for an automotive software infrastructure. Our work justifies how SDVs could be seen as a 'Data Center on Wheels', as Cloud Computing solves similar problems with different constraints. We identify required adaptations and promising technologies to fill the implementation gaps.
%     \item \textbf{In-vehicle communications (in progress):} We start by proposing an automated methodology to manage the high diversity of Quality-of-Service (QoS) network requirements despite the high number of upcoming services. We present our ongoing work in Section \ref{sec:paper}.
%     \item \textbf{Legacy communications:} Then, we plan to study the integration of \textit{legacy} (i.e. reused) ECUs into the upcoming SOA ecosystem for backwards compatibility. While these ECUs require the use of CAN networks, we will propose network virtualization and frame translation techniques to minimise latency and resource utilization.
%     \item \textbf{V2X communications:} Finally, with the increasing importance of connected services, we will study the interaction of in-vehicle and V2X communications.
% \end{enumerate}


% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{assets/iaas.pdf}
%     \caption{The Infrastructure-as-a-Service (IaaS) paradigm can be conceptually applied to both Cloud Native (left) and Automotive (right) environments. Physical servers or ECUs and network infrastructures can be abstracted as a unified platform for upper-layer application management middlewares.}
%     \label{fig:iaas}
% \end{figure}


% \section{State of the art}
% ZOA and SOA are expected to dynamically manage the lifecycle of all the onboard services during the vehicle lifetime. Figure \ref{fig:iaas} illustrates our main focus: we propose to define ZOA and SOA by following the Cloud Computing \textit{Anything-as-a-Service} (XaaS) paradigm, where resources are managed by independent subsystems and integrated into abstraction layers. We propose to classify the current literature into three layers.

% First, the \textbf{Hardware-as-a-Service} (HaaS) layer includes hardware virtualization management solutions that provision computing and peripheral resources to isolate independent services in shared ECUs. Virtualisation levels (mainly Virtual Machines and Containers) must be carefuly selected, configured and dynamically managed to run services in safe and secure environments while minimizing CPU and memory overhead.  Our survey reviews the most relevant strategies.

% Second, the \textbf{Network-as-a-Service} (NaaS) layer aims to transparently connect all services while respecting the flows' QoS requirements. Software Defined and Time Sensivite Networking (SDN and TSN) are promising technologies that offer dynamic routing and real-time communications in Ethernet networks \cite{hackelSoftwareDefined2019,hackelSecure2022}. However, several research directions must still be adressed such as legacy \& external network integration, dynamic (re)configuration, monitoring, and diagnostics.

% Finally, the \textbf{Infrastructure-as-a-Service} (IaaS) layer abstracts the previously mentionned layers into a unified and global view of the onboard resources. This layer includes \textit{control services} such as monitoring, self-healing, intrusion detection, online network scheduling, and global reconfiguration.

% Although not in the scope of this PhD, the SOA middleware then orchestrates the lifecycle of all embedded services and calls IaaS to both update and monitor the current vehicle state.

\section{Predictive network configuration} \label{sec:paper}

This work aims to automate the configuration of the entire in-vehicle network stack to guarantee all QoS requirements. In a SOA context, services will share the in-vehicle Ethernet backbone despite their highly diverse QoS requirements (e.g. best-effort for infotainment \textit{vs} time-sensitive motor control). Additionally, with the increase of user personalization, services will dynamically launch according to the user requests, vehicle context and OTA updates.

Currently, the automotive industry generates \textit{worst case} network schedules by including all services' flows into a static solution. However, the increasing number of services will make this strategy unpractical, as it would require high-bandwidth physical links even though the vehicle never runs all apps at the same time. Additionally, even though TSN is a promising solution for time-sensitive QoS control through the use of time-based traffic shaping, the configuration of the data plane is NP-hard. As a result, this strategy may soon become expensive in hardware, computationally infeasible, or both.

We propose to leverage the dynamic nature of ZOA and SOA by generating partitions of the global set of flows to obtain multiple smaller schedules. The vehicle then reconfigures the network based on the runtime context by selecting the correct pre-solved schedule using existing techniques \cite{hackelSecure2022}.

We model the vehicle states as a Markov chain where nodes contain a set of active apps and edge weights represent the transition frequency. We then model the TSN scheduling problem as an ILP programming problem. We are working on extending the open source TSNsched project \cite{santosTSNSCHED2019} to support the generation of multiple schedules while minimizing flow disruption between transitions, and maximizing best-effort bandwidth. Figure X presents a simple scheduling example.

We expect to submit our survey and obtain our first simulation results by September 2022. Next steps include the development of a physical test bench for further evaluation.
